Semantic Query Reformulation in Social PDMS

We consider social peer-to-peer data management systems (PDMS), where each peer maintains both semantic mappings between its schema and some acquaintances, and social links with peer friends. In this context, reformulating a query from a peer's schema into other peer's schemas is a hard problem, as it may generate as many rewritings as the set of mappings from that peer to the outside and transitively on, by eventually traversing the entire network. However, not all the obtained rewritings are relevant to a given query. In this paper, we address this problem by inspecting semantic mappings and social links to find only relevant rewritings. We propose a new notion of 'relevance' of a query with respect to a mapping, and, based on this notion, a new semantic query reformulation approach for social PDMS, which achieves great accuracy and flexibility. To find rapidly the most interesting mappings, we combine several techniques: (i) social links are expressed as FOAF (Friend of a Friend) links to characterize peer's friendship and compact mapping summaries are used to obtain mapping descriptions; (ii) local semantic views are special views that contain information about external mappings; and (iii) gossiping techniques improve the search of relevant mappings. Our experimental evaluation, based on a prototype on top of PeerSim and a simulated network demonstrate that our solution yields greater recall, compared to traditional query translation approaches proposed in the literature.

==> conclusion.tex <==
\section{Conclusions and Future Work}~\label{sec:concl}
In this paper, we have studied the problem of semantic query reformulation in 
social-based PDMS. We have presented a new notion of relevance of a query to a mapping and introduced a global metric for ordering the mappings considered in query rewriting. 
%By means of an extensive experimental analysis, we have proved the robustness of our approach. 
Future work is devoted to study the impact of query personalization, the combination with other quality metrics and the extension to unions of conjunctive queries (UCQs).


==> ref_report.tex <==
\begin{thebibliography}{10}

\bibitem{Aberer03}
K.~Aberer, P.~Cudr{\'e}-Mauroux, and M.~Hauswirth.
\newblock The chatty web: emergent semantics through gossiping.
\newblock In {\em WWW}, 2003.

\bibitem{Arenas2010}
M.~Arenas, J.~P{\'e}rez, J.L. Reutter, and C.~Riveros.
\newblock Foundations of schema mapping management.
\newblock In {\em PODS}, pages 227--238, 2010.

\bibitem{Arenas2008a}
M.~Arenas, J.~Pérez, and C.~Riveros.
\newblock {The Recovery of a Schema Mapping: Bringing Exchanged Data Back}.
\newblock In {\em {ACM PODS}}, pages 13--22, 2008.

\bibitem{Berners2009}
C.~Bizer, T.~Heath, and T.~Berners-Lee.
\newblock Linked data - the story so far.
\newblock {\em Int. J. Semantic Web Inf. Syst.}, 5(3):1--22, 2009.

\bibitem{Bloom70space}
B.H. Bloom.
\newblock Space/time trade-offs in hash coding with allowable errors.
\newblock {\em Communications of the ACM}, 13, 1970.

\bibitem{Bonifati2010}
A.~Bonifati, E.Q. Chang, T.~Ho, L.V.S. Lakshmanan, R.~Pottinger, and Y.~Chung.
\newblock Schema mapping and query translation in heterogeneous p2p xml
  databases.
\newblock {\em VLDB J.}, 19(2):231--256, 2010.

\bibitem{ang10}
Angela Bonifati, Ruilin Liu, and Hui~(Wendy) Wang.
\newblock Distributed and secure access control in p2p databases.
\newblock In {\em 24th Annual IFIP WG 11.3 Working Conference on Data and
  Applications Security and Privacy}, 2010.

\bibitem{Calvanese08}
D.~Calvanese, G.~De Giacomo, D.~Lembo, M.~Lenzerini, A.~Poggi, R.~Rosati, and
  M.~Ruzzi.
\newblock Data integration through dl-lite$_{\mbox{a}}$ ontologies.
\newblock In {\em SDKB}, 2008.

\bibitem{Fagin2007b}
R.~Fagin.
\newblock {Inverting Schema Mappings}.
\newblock {\em ACM TODS}, 32(4), 2007.

\bibitem{Fagin2009}
R.~Fagin, L.~M. Haas, M.~Hernandez, R.~J. Miller, L.~Popa, and Y.~Velegrakis.
\newblock {\em {Conceptual Modeling: Foundations and Applications}}, chapter
  {Clio: Schema Mapping Creation and Data Exchange}, pages 198--236.
\newblock Springer, 2009.

\bibitem{Fagin2005a}
R.~Fagin, P.G. Kolaitis, R.J. Miller, and L.~Popa.
\newblock {Data Exchange: Semantics and Query Answering}.
\newblock {\em TCS}, 336(1):89--124, 2005.

\bibitem{Fagin200589}
Ronald Fagin, Phokion~G. Kolaitis, RenÃ©e~J. Miller, and Lucian Popa.
\newblock Data exchange: semantics and query answering.
\newblock {\em Theoretical Computer Science}, 336(1):89 -- 124, 2005.

\bibitem{fan98}
L.~Fan, P.~Cao, J.M. Almeida, and A.Z. Broder.
\newblock Summary cache: A scalable wide-area web cache sharing protocol.
\newblock In {\em SIGCOMM}, pages 254--265, 1998.

\bibitem{Halevy05}
A.Y. Halevy, Z.G. Ives, D.~Suciu, and I.~Tatarinov.
\newblock Schema mediation for large-scale semantic data sharing.
\newblock {\em VLDB J.}, 14(1):68--83, 2005.

\bibitem{Ives2004}
Zachary~G. Ives, Alon~Y. Halevy, Peter Mork, and Igor Tatarinov.
\newblock Piazza: mediation and integration infrastructure for semantic web
  data.
\newblock {\em J. Web Sem.}, 1(2):155--175, 2004.

\bibitem{Kantere09}
V.~Kantere, D.~Tsoumakos, T.K. Sellis, and N.~Roussopoulos.
\newblock Groupeer: Dynamic clustering of p2p databases.
\newblock {\em Inf. Syst.}, 34(1):62--86, 2009.

\bibitem{miller03}
A.~Kementsietsidis, M.~Arenas, and R.J. Miller.
\newblock Mapping data in peer-to-peer systems: semantics and algorithmic
  issues.
\newblock In {\em {SIGMOD}}, pages 325--336, 2003.

\bibitem{KermarrecS07}
A.~Kermarrec and M.~van Steen.
\newblock Gossiping in distributed systems.
\newblock {\em Operating Systems Review}, 41(5):2--7, 2007.

\bibitem{Koloniari04}
G.~Koloniari and E.~Pitoura.
\newblock Content-based routing of path queries in peer-to-peer systems.
\newblock In {\em EDBT}, 2004.

\bibitem{Lenzerini2002}
M.~Lenzerini.
\newblock {Data integration: a Theoretical Perspective}.
\newblock In {\em {ACM PODS}}, pages 233--246, 2002.

\bibitem{Levy1995}
A.~Y. Levy, A.~O. Mendelzon, Y.~Sagiv, and D.~Srivastava.
\newblock {Answering Queries Using Views}.
\newblock In {\em PODS}, 1995.

\bibitem{peersim}
{T}he {Peersim} simulator.
\newblock \texttt{\scriptsize{http://peersim.sf.net}}.

\bibitem{Popa2002}
L.~Popa, Y.~Velegrakis, R.~J. Miller, M.~A. Hernandez, and R.~Fagin.
\newblock {Translating Web Data}.
\newblock In {\em {VLDB}}, 2002.

\bibitem{potti01}
R.~Pottinger and A.Y. Halevy.
\newblock Minicon: A scalable algorithm for answering queries using views.
\newblock {\em VLDB J.}, 10(2-3):182--198, 2001.

\bibitem{Yu2004}
C.~Yu and L.~Popa.
\newblock Constraint-based xml query rewriting for data integration.
\newblock In {\em {SIGMOD}}, 2004.

\end{thebibliography}

